Surface HOF: Surface Reconstruction from a Single Image Using Higher Order Function Networks

We address the problem of generating a high-resolution surface reconstruction from a single image. Our approach is to learn a Higher Order Function (HOF) which takes an image of an object as input and generates a mapping function. The mapping function takes samples from a canonical domain (e.g. the unit sphere) and maps each sample to a local tangent plane on the 3D reconstruction of the object. Each tangent plane is represented as an origin point and a normal vector at that point. By efficiently learning a continuous mapping function, the surface can be generated at arbitrary resolution in contrast to other methods which generate fixed resolution outputs. We present the Surface HOF in which both the higher order function and the mapping function are represented as neural networks, and train the networks to generate reconstructions of PointNet objects. Experiments show that Surface HOF is more accurate and uses more efficient representations than other state of the art methods for surface reconstruction. Surface HOF is also easier to train: it requires minimal input pre-processing and output post-processing and generates surface representations that are more parameter efficient. Its accuracy and convenience make Surface HOF an appealing method for single image reconstruction.

==> unused_text.tex <==


\paragraph{Cost function:} Chamfer + Stretch

Chamfer for object coverage

Stretch has two components: normals and Euclidean distance within a patch


\vtxt{In the future we might explore only one direction of chamfer for coverage}

\paragraph{Representative objects:} cube, torus, table

\paragraph{Results to show:}

train chamfer-only; chamfer+dist; chamfer+norm; chamfer+dist+norm

report: chamfer; dist; normal and total costs; maybe some other statistics related to stretch

Figures: reconstructions; normals (deviation from the ground truth); color visualizations of the preimage 
See Figure~\ref{fig:initial_results}



% There has been significant interest in moving away from fixed resolution object representatins such as voxel grids, or fixed cardinality points sets or graphs to continuous represenatations such as the signed distance function or a union of manifolds. 

% In this paper we present a new representation based on the fast weights paradigm where we ...


% \begin{itemize}
%     \item We address the problem of generating a 3D surface representing an object from a single image \vtxt{to-do: check 2d vs 3d surface terminology}
%     \item Why is it important to have a surface: for applications such as grasping (GraspIt requires surface input; not just a point cloud), visualization, rendering etc. 
%     \item We represent the surface as a mapping from the unit sphere to the object surface. Limitations of prior work are fixed resolution and hand tuning of domain parameters such as number of smooth surfaces covering the object and correspondences between them.
%     \item Highlights: resolution, simple triangulation, yields part decomposition, \vtxt{we hope}
% \end{itemize}



